Implicit Autoencoder for Point-Cloud Self-Supervised Representation Learning

This paper advocates the use of implicit surface representation in autoencoder-based self-supervised 3D representation learning. The most popular and accessible 3D representation, i.e., point clouds, involves discrete samples of the underlying continuous 3D surface. This discretization process introduces sampling variations on the 3D shape, making it challenging to develop transferable knowledge of the true 3D geometry. In the standard autoencoding paradigm, the encoder is compelled to encode not only the 3D geometry but also information on the specific discrete sampling of the 3D shape into the latent code. This is because the point cloud reconstructed by the decoder is considered unacceptable unless there is a perfect mapping between the original and the reconstructed point clouds. This paper introduces the Implicit AutoEncoder (IAE), a simple yet effective method that addresses the sampling variation issue by replacing the commonly-used point-cloud decoder with an implicit decoder. The implicit decoder reconstructs a continuous representation of the 3D shape, independent of the imperfections in the discrete samples. Extensive experiments demonstrate that the proposed IAE achieves state-of-the-art performance across various self-supervised learning benchmarks.

==> figures_tex/analysis.tex <==
\begin{figure*}[h]
    \centering
%\includegraphics[width=0.9\textwidth]{ICCV_2023/figures/compare.pdf}
    \begin{overpic}[width=0.9\linewidth]{figures/compare.pdf}
    \put(15,-1.5){(a)}
    \put(44,-1.5){(b)}
    \put(76,-1.5){(c)}
    \end{overpic}
    \vspace{5pt}
    \caption{\small{\textbf{Experiment analysis on Explicit and Implicit Autoencoders.} \textbf{(a)} T-SNE visualization for encoder latent codes of IAE (blue) and EAE (orange). The IAE clusters are noticeably smaller. \textbf{(b)} The average cluster radius for IAE and EAE in (a). \textbf{(c)} When increasing the input resolution, the performance gap between explicit and implicit models decreases.\protect\footnotemark. }}
    \label{fig:analysis}
    %%\vspace{-30pt}
\end{figure*}



==> figures_tex/completion.tex <==
\begin{figure}[t]
\begin{minipage}[b]{.46\linewidth}
    \centering
    \begin{tabular}{l|lc}
    \toprule
    Decoder & Method & SUN RGB-D \\
        \midrule
        \multirow{3}{*}{Explicit} &  FoldingNet~\cite{yang2018foldingnet} & 58.2 \\
        & OcCo~\cite{wang2020unsupervised} & 58.4  \\
        & SnowflakeNet~\cite{xiang2021snowflakenet} & 58.1 \\
        \midrule
        Implicit & Conv-OccNet~\cite{peng2020convolutional} &  \textbf{60.4} \\
        \bottomrule
    \end{tabular}
    \captionof{table}{\textbf{Comparison between explicit approaches and our model} on real data completion task. Our model built upon convolutional occupancy network shows consistent improvements.}
    \label{tab:complete_comp}
\end{minipage}\hspace{.02\lin ewidth}
\begin{minipage}[b]{.5\linewidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/completion.png}
    \caption{\textbf{Qualitative completion results on ScanNet.}  We show the results of SnowflakeNet~\cite{xiang2021snowflakenet} and our model.}
    \label{fig:complete}
\end{minipage}
%\vspace{-15pt}
\end{figure}

==> figures_tex/supp_compare.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/supp_teaser.pdf}
    \caption{\small{\textbf{Comparison between Explicit Autoencoder and Implicit Autoencoder}. Given a 3D shape, we randomly take two samples. For Implicit Autoencoder, we use 3D CAD model to represent the implicit function target for better visualization.}}
    \label{fig:supp_compare}
    \vspace{-10pt}
\end{figure}

==> figures_tex/tsne.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/tsne.pdf}
    \caption{\textbf{Visualization of learned features.} We visualize the learned features for each sample in ModelNet10 using t-SNE. All the models use DGCNN as the encoder backbone. (a) uses random initialization. (b), (c), (d) are pre-trained on ShapeNet.}
    \label{fig:tsne}
    %%\vspace{-2mm}
    %\vspace{-20pt}
\end{figure}

==> sections/05_discussion.tex <==
\section{Discussions}

\subsection{The difference between data augmentation and sampling variation.}

\subsection{Cases When Mesh Data Is Not Available}
\chen{This section provides little additional information. My suggestion is to remove it.}
An accurate implicit representation of 3D data is not generally available for real-world data since a continuous representation, e.g., a triangular mesh, is unavailable. To address this issue, we use the nearest neighbor strategy to estimate the unsigned distance label from the original point cloud(Sec~\ref{sec:setup}). The obtained implicit representations still suffer from imperfections and the sampling variation our method tries to avoid. However, compared to the traditional explicit autoencoder, which can only handle sub-sampled point clouds(1k$\sim$2k points), we argue that our work can still reduce this variation significantly because the implicit label is estimated from the original dense point cloud. The improved results in Sec~\ref{sec:tasks} provide the evidence. To further validate this claim, we conduct the same experiment as the second one in Section~\ref{sec:analysis}. This time we pretrain the IAE with an unsigned distance label from the original point cloud without using mesh. As shown in the Figure~\ref{fig:analysis} Right \textcolor[rgb]{0.0,0.0,1.0}{blue} line, even without mesh data to generate the accurate implicit values, the result is still very close to the IAE with mesh. This experiment validates that when the accurate implicit representation is not available, our model can still perform better than explicit autoencoders.

\subsection{Is it a fair comparison with previous approaches?}

==> tables/cls.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l|cc}
        \toprule
        \textbf{Method} & \textbf{\#points} & \textbf{Acc. (\%)} \\
        \midrule
        PointNet~\cite{qi2017pointnet++} & 1k & 89.2 \\
        PointNet++~\cite{qi2017pointnet} & 1k &  90.7 \\
        PointCNN~\cite{li2018pointcnn} & 1k & 92.2 \\
        KPConv~\cite{thomas2019kpconv} & 1k & 92.9 \\
        PointTransform~\cite{zhao2021point} & 1k & 93.7 \\
        PointNeXt~\cite{qian2022pointnext} & 1k & 93.2 \\
        PointMLP~\cite{ma2022rethinking} & 1k & 94.1 \\
        \midrule
        PointViT~\cite{yu2021point} & 1k & 91.4 \\
        $\text{[S]}$ Point-BERT~\cite{yu2021point} & 1K & 93.2 \\
        $\text{[S]}$Point-MAE~\cite{pang2022masked} & 1k & 93.8 \\
        $\text{[S]}$Point-MAE~\cite{pang2022masked} & 8k & \underline{94.0} \\
        DGCNN~\cite{wang2019dynamic} &  1k & 92.9 \\
        $\text{[S]}$FoldingNet~\cite{yang2018foldingnet}* & 1k & 93.1 \\
        $\text{[S]}$STRL~\cite{huang2021spatio}* & 1k & 93.1 \\
        $\text{[S]}$OcCo~\cite{wang2020unsupervised}* & 1k & 93.0 \\
        \rowcolor{gray!20} $\text{[S]}$IAE w/o mesh* & 1k & 94.0\\
        \rowcolor{gray!20} $\text{[S]}$IAE* & 1k & \textbf{94.2} \textcolor[rgb]{0,0.6,0}{(+1.2)} \\
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{\textbf{Shape classification fine-tuned results on ModelNet40.} Supervised methods train from scratch. Self-supervised methods(denoted by [S]) use the pre-trained models as the initial weight for supervised fine-tuning. `$\#$points' denotes number of input points. * methods use the same DGCNN encoder backbone. \textcolor[rgb]{0,0.6,0}{green} number shows the absolute improvement under the same backbone.}}
    \label{tab:mn40_ft}
\vspace{-0.1in}
\end{table}

==> tables/detection.tex <==
\begin{table*}[t]
    \centering
   \setlength\tabcolsep{20pt}% 调整列间距
    \begin{tabular}{l|cc|cc}
        \toprule
         & \multicolumn{2}{c}{\textbf{ScanNet}} & \multicolumn{2}{c}{\textbf{SUN RGB-D}} \\
        \textbf{Method} & $\textbf{AP}_{50}$ & $\textbf{AP}_{25}$ & $\textbf{AP}_{50}$ & $\textbf{AP}_{25}$ \\
        \toprule
        3D-MPA~\cite{engelmann20203d} & 49.2 & 64.2 & - & - \\
        MLCVNet~\cite{xie2020mlcvnet} & 41.4 & 64.5 & - & 59.8 \\
        H3DNet~\cite{zhang2020h3dnet} & 48.1 & 67.2 & 39.0 & 60.1 \\
        BRNet~\cite{cheng2021back} & 50.9 & 66.1 & 43.7 & 61.1 \\
        3DETR~\cite{misra2021end} & 47.0 & 65.0 & 32.7 & 59.1 \\
        GroupFree~\cite{liu2021group} & 52.8 & 69.1 & 45.2 & 63.0 \\
        \midrule
        VoteNet~\cite{qi2019deep}  &  33.5  & 58.6 & 32.9 & 57.7 \\
        %OcCo\cite{wang2020unsupervised} & 37.9 & 59.8 & 34.8 & 59.6 \\
        $\text{[S]}$ STRL\cite{huang2021spatio} & 38.4 & 59.5 & 35.0 & 58.2 \\
        $\text{[S]}$ RandomRooms\cite{rao2021randomrooms} & 36.2 & 61.3 & 35.4 & 59.2 \\
        $\text{[S]}$ PointContrast\cite{xie2020pointcontrast} & 38.0 & 59.2 & 34.8 & 57.5 \\
        $\text{[S]}$ DepthContrast\protect\footnotemark \cite{zhang2021self} & 39.1 & \textbf{62.1} & 35.4 & \textbf{60.4}\\
        %DepthContrast($3\times$; \text{both}) & 42.9 & 64.0 \\
        \rowcolor{gray!20} $\text{[S]}$ IAE & \textbf{39.8} & 61.5 & \textbf{36.0} & \textbf{60.4} \\
        \midrule
        FCAF3D~\cite{rukhovich2021fcaf3d} & 57.3 & 71.5 & 48.9 & 64.2 \\
        \rowcolor{gray!20} $\text{[S]}$ IAE(FCAF3D) & \textbf{58.6}\textcolor[rgb]{0,0.6,0}{(+1.3)} & \textbf{72.5}\textcolor[rgb]{0,0.6,0}{(+1.0)} & \textbf{50.0}\textcolor[rgb]{0,0.6,0}{(+1.1)} & \textbf{65.0}\textcolor[rgb]{0,0.6,0}{(+0.8)} \\
        \bottomrule
    \end{tabular}
    \caption{\small{\textbf{3D object detection results.} We fine-tune our pre-trained model on ScanNetV2 and SUN-RGBD validation set using VoteNet~\cite{qi2019deep} and FCAF3D~\cite{rukhovich2021fcaf3d}. We show mean of average precision~(mAP) across all semantic classes with 3D IoU threshold 0.25 and 0.5. [S] denotes the self-supervised methods. Our method outperforms prior work across most metrics.}}
    \label{tab:detection}
%%\vspace{-7mm}
\end{table*}

==> tables/diff_aug_3.tex <==
\begin{table}[t]
    \centering
   %\setlength\tabcolsep{6pt}% 调整列间距
   %\renewcommand\arraystretch{1.1}
   %\vspace{-15pt}
    \begin{tabular}{c|ccccc}
        \toprule
        Aug & scratch & cr=0 & cr=20\% & cr=50\%& cr=70\% \\
        \hline
        SUN & 57.7 & 60.0 & 60.2 & \textbf{60.4} & 59.8 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Different setting of scene data augmentation.} `cr' denotes max cropping ratio. `scratch' means training from scratch.}
    \label{tab:data_aug}
\end{table}

==> tables/seg.tex <==
\begin{table}[t]
    \setlength\tabcolsep{11pt}
    \centering
    \begin{tabular}{l|ll}
        \toprule
        \textbf{Method} & \textbf{OA} & \textbf{mIoU} \\
        \midrule
        PointNet & 78.5 & 47.6 \\
        PointCNN & 88.1 & 65.4 \\
        DGCNN~\cite{wang2019dynamic} & 84.1 & 56.1 \\
        KPConv & - & 70.6 \\
        PointTransformer & 90.2 & 73.5 \\
        \midrule
        $\text{[S]}$Jigsaw~\cite{sauder2019self} & 84.4 & 56.6 \\
        $\text{[S]}$OcCo~\cite{wang2020unsupervised} & 85.1 & 58.5 \\
        \rowcolor{gray!20} $\text{[S]}$IAE & \textbf{85.9}\textcolor[rgb]{0,0.6,0}{(+0.8)} & \textbf{60.7}\textcolor[rgb]{0,0.6,0}{(+2.2)} \\
        \midrule
        PointNeXt~\cite{qian2022pointnext} & 90.3 & 74.9 \\
        \rowcolor{gray!20} $\text{[S]}$ IAE(PointNeXt) & \textbf{90.8}\textcolor[rgb]{0,0.6,0}{(+0.5)} & \textbf{75.3}\textcolor[rgb]{0,0.6,0}{(+0.4)} \\
        
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{\textbf{Semantic segmentation results on S3DIS 6-Fold.} We show overall accuracy~(OA) and mean intersection of union~(mIoU) across six folds.}}
    \label{tab:semseg}
\end{table}

==> tables/svm.tex <==
\begin{table}[h]
    %\resizebox{\textwidth}{20mm}
    \centering
    \setlength\tabcolsep{25pt}
    \begin{tabular}{l|c}
        \toprule
        \textbf{Method} & \textbf{Acc. (\%)} \\
        \midrule
        %Random &  60.2\% \\
        3D-GAN~\cite{wu2016learning}  & 83.3 \\
        Latent-GAN~\cite{achlioptas2018learning} & 85.7 \\
        SO-Net~\cite{li2018so} & 87.3 \\
        MAP-VAE~\cite{han2019multi} & 88.4 \\
        Point-BERT~\cite{yu2021point} & 87.4 \\
        Point-MAE~\cite{pang2022masked} & 88.5 \\
        \midrule
        Jigsaw~\cite{sauder2019self}$^*$ & 84.1 \\
        FoldingNet~\cite{yang2018foldingnet}$^*$ & 90.1 \\
        Orientation~\cite{poursaeed2020self}$^*$ & 90.7 \\
        STRL~\cite{huang2021spatio}$^*$ & 90.9 \\
        OcCo~\cite{wang2021unsupervised}$^*$ & 89.7 \\
        CrossPoint~\cite{afham2022crosspoint} $^*$ & 91.2 \\
        \rowcolor{gray!20} IAE w/o mesh$^*$ & 91.7 \\
        \rowcolor{gray!20} IAE$^*$ & \textbf{92.1} \textcolor[rgb]{0,0.6,0}{(+0.9)} \\
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{\textbf{Linear evaluation for shape classification on ModelNet40}. For fair comparisons, different $^*$ methods use the same DGCNN encoder backbone. \textcolor[rgb]{0,0.6,0}{green} number shows the absolute improvement.}}
    \label{tab:mn40}
%\vspace{-0.1in}
\end{table}
